Reducing Redundant Work in Jump Point Search

JPS (Jump Point Search) is a state-of-the-art optimal algorithm for online grid-based pathfinding. Widely used in games and other navigation scenarios, JPS nevertheless can exhibit pathological behaviours which are not well studied: (i) it may repeatedly scan the same area of the map to find successors; (ii) it may generate and expand suboptimal search nodes. In this work, we examine the source of these pathological behaviours, show how they can occur in practice, and propose a purely online approach, called Constrained JPS (CJPS), to tackle them efficiently. Experimental results show that CJPS has low overheads and is often faster than JPS in dynamically changing grid environments: by up to 7x in large game maps and up to 14x in pathological scenarios.

==> algos/alg_retrieve.tex <==
\caption{Bidirectional path extraction at runtime for an ($s,t)$ pair}
\label{alg:wild}
$\mbox{prefix} \gets []$ \\
$\mbox{suffix} \gets []$ \\
\While{$s \neq t$}
      {\eIf{$(s,t) \in R$}
           {$(s,n) \gets$ \textsf{FirstMove}($s,t$) \\
             $\mbox{prefix} \gets \mbox{prefix} \pp [(s,n)]$ \\
             $s \gets n$ }
           {$(t,n) \gets$ \textsf{FirstMove}($t$,$s$) \\
             $\mbox{suffix} \gets [(n,t)] \pp \mbox{suffix}$ \\
        $t \gets n$}
      }
\Return $\mbox{prefix} + \mbox{suffix}$


==> algos/astar.tex <==
\SetKwInput{Input}{Variables}
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{OctileDistance}{OctileDistance}

\Input{\\
  $open$: the priority queue; \\
  $f$: table for the f-value of all vertices; \\
  $g$: table for the g-value of all vertices; \\
}

\lFor{$n \in V$}{$g[n] \gets \infty$}
$open \gets \{s\}$;\\
$g[s] \gets 0$;\\ 
$f[s] \gets 0$; \\
\While{$open \neq \emptyset$} {
  $n \gets \argmin \{ f[n']~|~n' \in open\}$ \\
  $open \gets open - \{n\}$;\\
  \lIf{$n == t$}{\Return $g[n]$}
  \For{$(n,m) \in E$} {
    \If{$g[n] + w(n, m) < g[m]$} {
      $g[m] \gets g[n] + w(n, m)$;\\
      $f[m] \gets g[m] + Heuristic(m, t)$; \\
      $open \gets open \cup \{m\}$;\\
    }
  }
}

\Return $\bot$   \hfill $\blacktriangleright$ No solution


==> algos/backwards_scan.tex <==
\SetKwInput{Input}{Input}
\SetKwFunction{boundedScan}{boundedScan}
\Input{
  $a$: the starting location of the scanning;\\
  $n$: the location of the found jump point; \\
  $d$: the direction of the scanning;\\
  $db$: the bit map for block based scanning; \\
\boundedScan{$C, D, L, db$} {
  {:} Algorithm~\ref{alg:jumplimit}
}
}
$cnt \gets 0$;\\
$c \gets n$;\\
\While{$c \neq a$ and $cnt \leq 2$}{
  \tcp{scan from c in the reverse direction and not cross a}
  $p \gets \textsf{boundedScan}(c, -d, |ac|, db)$;\\ 
  $g_p \gets \min\{g_p, g_a + |ap|\}$; \\
  $c \gets p$; \\
  $cnt \gets cnt + 1$;\\
}


==> algos/bidirectional.tex <==
$\mbox{prefix} \gets []$ \\
$\mbox{suffix} \gets []$ \\
\While{$s \neq t$}
      {\eIf{$(s,t) \in R$}
           {$(s,n) \gets$ \textsf{CPD}($s,t$) \\
             $\mbox{prefix} \gets \mbox{prefix} + [(s,n)]$ \\
             $s \gets n$ }
           {$(t,n) \gets$ \textsf{CPD}($t$,$s$) \\
             $\mbox{suffix} \gets [(n,t)] + \mbox{suffix}$ \\
        $t \gets n$}
      }
\Return $\mbox{prefix} + \mbox{suffix}$


==> algos/branchless_jlimit.tex <==
\SetKwInput{Input}{Input}
\SetKwFunction{scanning}{scanning}
\Input{
$C$: the current location (as a bit address); \\
$D$: the cardinal direction (as a bit delta, e.g. W = $-1$, E = $+1$, S = $+mw$, N = $-mw$ where $mw$ is the width of the map); \\
$L$: jump limit;\\
$db$: bit map for block based scanning ($1$ means obstacle) \\
\scanning{$C, D, db$} {
  {:} block-based scanning in~\cite{dblp:conf/aips/haraborg14} 
}
}
\tcp{store the original value in tmp}
$tmp \gets db(C+L\times D)$; \\
$db(C+L\times D) \gets 1$; \\
$\textsf{scanning}(C, D, db)$; \\ 
$db(C+L\times D) \gets tmp$;


==> algos/heur_encode_decode.tex <==
\SetKwProg{Fn}{Function}{:}{}
\SetKwFunction{Decode}{Decode}
\SetKwFunction{Encode}{Encode}


\Fn{\Encode{s, t}}{
  \If{$F_x$(s, t) $\in$ $T_s$[t])}{ $T_s$[t] = $T_s$[t] $\cup$ \heur\; }
}

\Fn{\Decode{m, s, t}} {
  \If{m = \heur} {
    \Return $F_x$(s, t)\;
  } \Else {
    \Return m\;
  }
}


==> algos/push_interval.tex <==
\SetKwInput{Input}{Input}
\Input{
  $I=(r, [xl, xu])$: the horizontal interval at the South border ($y=r.yu$) of rectangle $r$\\
  $Q$: the FIFO queue \\
}
$Q$.push($I$); \\
\While{$Q$ not empty}{
  $c \gets Q$.pop(); \\
  \tcp{Using the original JPS scanning on xl and xu}
    \tcp{Shrink the interval when find the jump point}
  \If{\textsf{ScanNorth}(xl, r.yu)} {
    xl=xl+1;\\
  }

  \If{\textsf{ScanNorth}(xr, r.yu)} {
    xr=xr-1;\\
  }

  \If{xl $\leq$ xr} {
    \tcp{Generate new interval adjacent to the north border}
    \For{adjr in NorthAdj(r.yl, xl, xr)}{
      $Q$.push((adjr, [adjr.xl, adjr.xu]));
    }
  }
}


==> algos/unidirectional.tex <==
$p \gets []$ \\
\While{$s \neq t$}
      {$(s,n) \gets$ \textsf{CPD}($s,t$) \\
       $p \gets p + [(s,n)]$ \\ 
       $s \gets n$
      }
\Return $p$


==> code/branchless_jlimit.tex <==
\SetKwInput{Input}{Input}
\Input{
$C$: the current location (as a bit address); \\
$D$: the cardinal direction (as a bit delta, e.g. W = $-1$, E = $+1$, S = $+mw$, N = $-mw$ where $mw$ is the width of the map); \\
$L$: jump limit;\\
$db$: bit map for block based scanning ($1$ means obstacle)
}

\tcp{store the original value in tmp}
$tmp \gets db(C+L\times D)$; \\
$db(C+L\times D) \gets 1$; \\
$block\_based\_scanning(C, D, db)$; \\
$db(C+L\times D) \gets tmp$;


==> src/2d-symmetric.tex <==
\matrix(m)[matrix of nodes,
    column sep=-\pgflinewidth, row sep=-\pgflinewidth,
    nodes in empty cells,
    nodes={draw,
      ultra thin,
      black!90,
      minimum height=0.8cm,
      anchor=center,
      text width=0.8cm,
      align=center,
      inner sep=0pt
    }] {
 & & & \\
 & & & \\
 & & & \\
};
\tikzstyle{nd}=[circle,fill=blue!40, inner sep=0pt, minimum size=4mm]
\coordinate (s) at (m-3-1);
\coordinate (t) at (m-1-4);

\newcommand{\drawnode} {
  \node[nd] at (s) {s};
  \node[nd] at (t) {t};
}

\newcommand{\drawpath} {
  \draw[-, very thick, shorten <= 7pt] (s.center) -- (m-1-3.center);
  \draw[->,very thick, shorten >= 5pt] (m-1-3.center) -- (t.center);

  \draw[-, very thick] (m-2-2.center) -- (m-2-3.center);
  \draw[->,very thick, shorten >= 5pt] (m-2-3.center) -- (t.center);

  \draw[-, very thick, shorten <= 7pt] (s.center) -- (m-3-2.center);
  \draw[->,very thick, shorten >= 5pt] (m-3-2.center) -- (t.center);
}

\newcommand{\drawlabel} {
  \node[label={[shift={(0, -0.2)}]$v_1$}, left] at (m-2-2) {};
  \node[label={[shift={(0, -0.2)}]$v_2$}, left] at (m-1-3) {};
  \node[label={[shift={(0, -0.55)}]$v_3$}, right] at (m-3-2) {};
  \node[label={[shift={(0, -0.55)}]$v_4$}, right] at (m-2-3) {};
}
\drawnode
\drawpath
\drawlabel


==> src/alg_astar.tex <==
\begin{algorithm}[t]
  \caption{ \textsf{Oracle-Search}($w,s,t,\epsilon$): 
   %Variant of Weighted A*  with an oracle. 
  Parameters $s$ and $t$ indicate the start and target, 
  $w$ encodes actual edge-costs.
  $O$ is the shortest path oracle. The \textsf{fst} function returns the first argument of a tuple.
  This algorithm guarantees solutions are $\epsilon$-optimal.
  \label{alg:retrieve}}
  $closed \gets \emptyset$;  $open \gets \{ s\}$ \\
  \lFor{$n \in N$}{$g[n] \gets \infty$}
  $g[s] \gets 0$; $f[s] \gets 0$; $p[s] \gets []$ \\
  $u \gets \infty$; $I \gets s$ \\
  
  \While{$open \neq \emptyset$}{
    $n \gets \argmin \{ f[n']~|~n' \in open \}$ \label{l:sn} \\
    \lIf{$n = t$}{\Return $p[n]$ \label{l:rn}}
        \lIf{$\epsilon f[n] \geq u$}
           {\Return $p[I] \pp{} \textsf{fst}~ O(I,t)$ \label{l:u}}
          $open \gets open - \{n\}$ \\
          $closed \gets closed \cup \{n\}$ \\
          \For{$(n,m) \in E, m \not\in closed$}
              {\If{$g[n] + w(n,m) < g[m]$}
                  {
		   %$open \gets open \cup \{m\}$ \\
                   $p[m] \gets p[n] \pp~ [(n,m)]$ \\
                   $g[m] \gets g[n] + w(n,m)$ \\
                   $\langle \pi, lb, ub\rangle \gets O(m,t)$ \label{l:wcpd} \\
                   $f[m] \gets g[m] + lb$ \label{l:f} \\ 
                    \If%{$f[m] < u$}
                       {$u > g[m] + ub \label{l:ub}$}
                       {$u \gets g[m] + ub$; $I \gets m$ \label{l:new}}
		   $open \gets open \cup \{m\}$ \\
                  }
              }
        }      
   \Return $\bot$   \hfill $\blacktriangleright$ No solution
\end{algorithm}



==> src/jps-constraint.tex <==
\tikzstyle{jp}=[circle,fill=blue!50, inner sep=0pt, minimum size=4mm]
\tikzstyle{jp2}=[circle,fill=green!90, inner sep=0pt, minimum size=4mm]
\tikzstyle{md}=[circle,fill=cyan!50, inner sep=0pt, minimum size=4mm]
\matrix(m)[
    matrix of nodes,
    nodes={draw,
      black!80,
      ultra thin,
      minimum height=0.8cm,
      anchor=center,
      minimum width=0.8cm,
      align=center,
      inner sep=0pt
    },
    column sep=-\pgflinewidth, 
    row sep=-\pgflinewidth,
    nodes in empty cells, 
] {
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
  & & & & & & & & & & & & & &\\
};
\coordinate (b) at (m-1-3);
\coordinate (a) at (m-13-3);
\coordinate (x) at (m-6-6);
\coordinate (y) at (m-8-6);
\coordinate (pm) at (m-7-3);
\coordinate (pd) at (m-7-9);
\coordinate (r1) at (m-4-15);
\coordinate (r2) at (m-10-15);

\newcommand{\drawObs}{
    \node[fill=black, inner sep=0pt, fit=(m-2-2)(m-12-2)] {}; 
    \node[fill=black, inner sep=0pt, fit=(m-7-5)] {}; 
    \node[fill=black, inner sep=0pt, fit=(m-5-14)(m-9-14)] {}; 
    % \node[fill=black, inner sep=0pt, fit=(m-1-9)(m-5-9)] {};
    % \node[fill=black, inner sep=0pt, fit=(m-9-9)(m-13-9)] {};
}

\newcommand{\drawNodes}{
    \node[jp] at (a) {$a$};
    \node[jp] at (x) {$x$};
    \node[jp2] at (b) {$b$};
    \node[jp2] at (y) {$y$};
    \node[md] at (pm) {$m$};
    \node[md] at (pd) {$d$};
    \node[jp] at (r1) {$r_1$};
    \node[jp2] at (r2) {$r_2$};
}

\newcommand{\drawScan}{
    \draw[->, very thick, black, shorten >=5pt] (m-1-1.center) -- (b.center);
    \draw[->, very thick, black, shorten >=5pt] (m-1-1.center) -- (b.center);
    \draw[->, very thick, green!70!black, shorten >=5pt] (b) -- (m-13-15.south east);
    \draw[->, very thick, black, shorten >=5pt] (m-13-1.center) -- (a.center);
    \draw[->, very thick, blue!80, shorten >=5pt] (a) -- (m-1-15.north east);
    
    \draw[->|, very thick, blue!80, shorten >=7pt] ([xshift=-2pt]a) -- ([xshift=-2pt]b); 
    \draw[->|, very thick, blue!80, shorten >= 1pt] (m-11-5.center) -- (m-8-5.north);
    \draw[->|, very thick, blue!80, shorten >=7pt, shorten <= -2pt] ([xshift=-2pt]m-10-6.center) -- ([xshift=-2pt]x); 
    \draw[->|, very thick, blue!80, shorten >=6pt] (m-4-12.center) -- (r1); 
    
    \draw[->|, very thick, green!70!black, shorten >=7pt,] ([xshift=2pt]b) -- ([xshift=2pt]a); 
    \draw[->|, very thick, green!70!black, shorten >= 1pt] (m-3-5.center) -- (m-6-5.south);
    \draw[->|, very thick, green!70!black, shorten >=7pt, shorten <= 2pt] ([xshift=2pt]m-4-6.center) -- ([xshift=2pt]y); 
    \draw[->|, very thick, green!70!black, shorten >=6pt] (m-10-12.center) -- (r2); 
}

\newcommand{\drawConstraint}{
    \begin{scope}[on background layer]
        \node[fill=yellow!30, inner sep=0pt, fit=(m-1-3)(m-1-4)]{};
        \node[fill=yellow!30, inner sep=0pt, fit=(m-7-3)(m-7-4)]{};
        \node[fill=yellow!30, inner sep=0pt, fit=(m-8-6)(m-8-8)]{};
        \node[fill=gray!30, inner sep=0pt, fit=(m-1-5)(m-6-5)]{};
        \node at (m-1-5) {?};

        \node[fill=red!20, inner sep=0pt, fit=(m-1-9)(m-13-15)]{};
    \end{scope}
    \draw[|<->|, shorten <=5pt, shorten >=1pt] (pm.center)--(m-7-4.east);
    \draw[|<->|, shorten <=5pt, shorten >=1pt] (b.center)--(m-1-4.east);
    \draw[|<->|, shorten <=5pt, shorten >=1pt] (y.center)--(m-8-8.east);
    \node[label={[shift={(0, -0.25)}]$c_b$}, above] at (m-1-4) {};
    \node[label={[shift={(0, -0.25)}]$c_m$}, above] at (m-7-4) {};
    \node[label={[shift={(0.2, -0.3)}]$c_y$}, above] at (m-8-7) {};
    \node[label={[shift={(0.05, -0.6)}]$a_1$}, right] at (m-12-4) {};
    \node[label={[shift={(0.05, -0.6)}]$a_2$}, right] at (m-11-5) {};
    \node[label={[shift={(0.05, -0.6)}]$a_3$}, right] at (m-10-6) {};
    \node[label={[shift={(0.05, -0.6)}]$a_4$}, right] at (m-9-7) {};
    \node[label={[shift={(0.05, -0.6)}]$a_5$}, right] at (m-8-8) {};
    \node[label={[shift={(-0.05, 0.6)}]$a_6$}, left] at (m-7-10) {};
    \node[label={[shift={(-0.05, 0.6)}]$a_7$}, left] at (m-6-11) {};
}

\drawObs
\drawScan
\drawNodes
\drawConstraint


==> src/jps-jumping.tex <==
\tikzstyle{jp}=[circle,fill=blue!40, inner sep=0pt, minimum size=4mm]
\tikzstyle{jp2}=[circle,fill=green!90, inner sep=0pt, minimum size=4mm]
\tikzstyle{pm}=[circle,fill=cyan!50, inner sep=0pt, minimum size=4mm]
\matrix(m)[
    matrix of nodes,
    row 1/.append style={nodes={draw=none}},
    column 1/.append style={nodes={draw=none}},
    column sep=-\pgflinewidth, row sep=-\pgflinewidth,
    nodes in empty cells,
    nodes={draw,
      ultra thin,
      black!90,
      minimum height=0.8cm,
      anchor=center,
      text width=0.8cm,
      align=center,
      inner sep=0pt
    }] {
  $y\backslash x$ &1&2&3&4&5&6&7\\
      1& & & & & & & \\
      2& & & & & & & \\
      3& & & & & & & \\
      4& & & & & & & \\
      5& & & & & & & \\
      6& & & & & & & \\
      7& & & & & & & \\
      % 8& & & & & & & & \\
      % 9& & & & & & & & \\
};

\newcommand{\constraint} {
  \node (b) at (m-4-8) [jp2] {\textbf{b}};
  \node (a) at (m-4-2) [jp] {\textbf{a}};
  \node (x) at (m-7-7) [jp2] {\textbf{x}};
    
  \draw[->,  very thick, black, shorten >=5pt] (m-2-2.center) -- (a.center);
  \draw[->,  very thick, black, shorten >=5pt] (m-2-8.center) -- (b.center);
  \draw[->,  very thick, blue!80, shorten >=5pt] (a) -- (m-8-6.south east);
  \draw[->|, very thick, blue!80, shorten >=7pt] (a) -- (b.center);
  \draw[->|, very thick, blue!80, shorten >=6pt] (m-7-5.center) -- (x.center);
  \draw[->|, very thick, blue!80, shorten >=1pt] (m-5-3.center) -- (m-5-5.west);
  \draw[dashed, ->|, very thick, blue!80, shorten >=1pt] (m-5-3.center) -- (m-5-8.west);
  \draw[->|, very thick, blue!80, shorten >=1pt] (m-6-4.center) -- (m-6-6.west);
  \draw[->|, very thick, green!70!black, shorten >=2pt, shorten <=6pt] (b.center) -- (m-5-7.south west);
  \draw[->|, very thick, green!70!black, shorten >=6pt] (m-5-7.center) -- (x.center);
  
  \node (d) at (m-4-5) [pm] {$m_1$};
  \node (e) at (m-7-6) [pm] {$m_2$};

  \draw[|<->|,  shorten <= 5pt, shorten >= 2pt] (b.center) -- (m-5-8.south);
  \node[label={[shift={(0.1, -0.3)}]$c_1'$}, right] at (m-5-8) {};
  
  \draw[|<->|,  shorten <= 5pt, shorten >= 2pt] (d.center) -- (m-5-5.south);
  \node[label={[shift={(0.1, -0.2)}]$c_1$}, right] at (m-5-5) {};
  
  \draw[|<->|,  shorten <= 5pt, shorten >= 2pt] (e.center) -- (m-8-6.south);
  \node[label={[shift={(-0.45, -0.2)}] $c_2$}, left] at (m-8-7) {};
  
  \node[label={[shift={(0.1, -0.3)}]$a_1$}, right] at (m-5-2) {};
  \node[label={[shift={(0.1, -0.3)}]$a_2$}, right] at (m-6-3) {};
  \node[label={[shift={(0.1, -0.3)}]$a_3$}, right] at (m-7-4) {};
  \node[label={[shift={(0.1, -0.3)}]$a_4$}, right] at (m-8-5) {};
  % \node[label={[shift={(0.1, -0.3)}]$a_5$}, right] at (m-9-6) {};
  % \node[label={[shift={(0.1, -0.3)}]$a_6$}, right] at (m-10-7) {};

  \begin{scope}[on background layer]
    \node[fill=black, inner sep=0pt, fit=(m-3-3)(m-3-7)]{};
    \node[fill=black, inner sep=0pt, fit=(m-6-6)] {};
    \node[fill=yellow!30, inner sep=0pt, fit=(m-4-8)(m-5-8)] {};
    \node[fill=yellow!30, inner sep=0pt, fit=(m-4-5)(m-5-5)] {};
    \node[fill=yellow!30, inner sep=0pt, fit=(m-7-6)(m-8-6)] {};
    \node[fill=gray!50, inner sep=0pt, fit=(m-6-7)(m-6-8)] {};
    \node at (m-6-8) {?};
  \end{scope}
}


==> src/jps-scanning.tex <==
\tikzstyle{jp}=[circle,fill=blue!40, inner sep=0pt, minimum size=4mm]
\tikzstyle{jp2}=[circle,fill=green!90, inner sep=0pt, minimum size=4mm]
\tikzstyle{pm}=[circle,fill=cyan!50, inner sep=0pt, minimum size=4mm]
\matrix(m)[square matrix] {
  & & & & & & & \\
  & & & & & & & \\
  & & & & & & & \\
  & & & & & & & \\
  & & & & & & & \\
  & & & & & & & \\
};

\newcommand{\defcoord} {
  \coordinate (a) at (m-6-3);
  \coordinate (x) at (m-2-5);
  \coordinate (y) at (m-2-3);
}

\newcommand{\drawObs} {
  \begin{scope}[on background layer]
    \node[fill=black, inner sep=0pt, fit=(m-1-2)(m-5-2)]{};
    \node[fill=black, inner sep=0pt, fit=(m-3-4)] {};
  \end{scope}
}

\newcommand{\scanA} {
  \defcoord
  \drawObs

  \draw[->,  very thick, shorten >=5pt] (m-6-1.center) -- (a);
  \draw[->,  very thick, blue!80, shorten >=5pt] (a) -- (m-1-8.north east);
  \draw[->|, very  thick, blue!80, shorten >=7pt] (a) -- (m-2-3.center);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-5-4.center) -- (m-4-4.north);
  \draw[->|, very  thick, blue!80, shorten >=7pt] (m-4-5.center) -- (x.center);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-3-6.center) -- (m-1-6.north);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-2-7.center) -- (m-1-7.north);
  \draw[->,  very thick, blue!80, shorten >=5pt] (a.center) -- (m-6-8.east);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-5-4.center) -- (m-5-8.east);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-4-5.center) -- (m-4-8.east);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-3-6.center) -- (m-3-8.east);
  \draw[->,  very thick, blue!80, shorten >=5pt] (m-2-7.center) -- (m-2-8.east);
  %
  \node[label={[shift={(-0.1, -0.2)}]$\mathbf{a_1}$}, left] at (m-5-4) {};
  \node[label={[shift={(-0.1, -0.2)}]$\mathbf{a_2}$}, left] at (m-4-5) {};
  \node[label={[shift={(-0.1, -0.2)}]$\mathbf{a_3}$}, left] at (m-3-6) {};
  \node[label={[shift={(-0.1, -0.2)}]$\mathbf{a_4}$}, left] at (m-2-7) {};
  \node[label={[shift={(-0.1, -0.2)}]$\ldots$}, left] at (m-1-8) {};
  %
  % % draw nodes
  \node[jp] at (a) {\textbf{a}};
  \node[jp] at (x) {$\mathbf{x_2}$};
  \node[jp] at (y) {$\mathbf{x_1}$};
}


==> src/pathological-ep.tex <==
\matrix(m)[coord matrix]{
  $y \backslash x$  & 1& 2& 3& 4& 5\\
  1 &  &  &  &  & \\
  2 &  &  &  &  & \\
  3 &  &  &  &  & \\
  4 &  &  &  &  & \\
  5 &  &  &  &  & \\
};

\newcommand{\drawEmpty} {
  \tikzstyle{n}=[circle,fill=gray!50, inner sep=0pt, minimum size=4mm]
  \coordinate (a) at (m-6-2);
  \draw[->, very thick, blue!70, shorten >=-10pt] (a) -- (m-2-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (a) -- (m-2-2.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-5-3.center) -- (m-2-3.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-4-4.center) -- (m-2-4.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-3-5.center) -- (m-2-5.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (a) -- (m-6-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-5-3.center) -- (m-5-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-4-4.center) -- (m-4-6.center);
  \draw[->, very thick, blue!70] (m-3-5.center) -- (m-3-6.east);
  \node[n] at (a) {\textbf{a}};
}

\newcommand{\drawCaseOne} {
  \begin{scope}[on background layer]
    \node[fill=black, inner sep=0pt, fit=(m-3-3)(m-4-4)]{};
  \end{scope}

  \coordinate (s) at (m-2-2);
  \coordinate (a) at (m-5-5);

  \tikzstyle{n}=[circle,fill=gray!50, inner sep=0pt, minimum size=4mm]

  \draw[-,  very thick, green!70!black] (s) -- (m-2-5.center);
  \draw[->, very thick, green!70!black, shorten >=5pt] (m-2-5.center) -- (a);
  \draw[->, very thick, green!70!black] ([yshift=-3pt]a) -- ([yshift=-3pt]m-5-4.center);
  \draw[->, very thick, green!70!black] (a) -- (m-6-5.center);
  \draw[->, very thick, green!70!black] (a) -- (m-6-4.center);

  \draw[-,  very thick, blue!70] (s) -- (m-5-2.center);
  \draw[->, very thick, blue!70, shorten >=5pt] (m-5-2.center) -- (a);
  \draw[->, very thick, blue!70] ([xshift=3pt]a) -- ([xshift=3pt]m-4-5.center);
  \draw[->, very thick, blue!70] (a) -- (m-5-6.center);
  \draw[->, very thick, blue!70] (a) -- (m-4-6.center);
  \draw[->, very thick, gray!70!black] (a) -- (m-6-6.center);


  \node[n] at (s) {\textbf{s}};
  \node[n] at (a) {\textbf{a}};
}

\newcommand{\drawCaseTwo} {

  \begin{scope}[on background layer]
    \node[fill=black, inner sep=0pt, fit=(m-4-2)(m-5-2)]{};
  \end{scope}

  \tikzstyle{n}=[circle,fill=gray!50, inner sep=0pt, minimum size=4mm]
  \coordinate (a) at (m-6-3);
  \draw[->, very thick, blue!70, shorten >=-10pt] (a) -- (m-3-6.center);
  \draw[->|, very thick, blue!70] (a) -- (m-3-3.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-5-4.center) -- (m-2-4.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-4-5.center) -- (m-2-5.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-3-6.center) -- (m-2-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (a) -- (m-6-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-5-4.center) -- (m-5-6.center);
  \draw[->, very thick, blue!70, shorten >=-10pt] (m-4-5.center) -- (m-4-6.center);
  \draw[->, very thick, blue!70] (m-3-6.center) -- (m-3-6.east);
  % \draw[->, thick] (m-2-2.center) -- (m-6-2.center);
  % \draw[->, thick] (m-3-3.center) -- (m-6-3.center);
  % \draw[->, thick] (m-4-4.center) -- (m-6-4.center);
  % \draw[->, thick] (m-5-5.center) -- (m-6-5.center);
  % \draw[->, thick] (m-2-2.center) -- (m-2-6.center);
  % \draw[->, thick] (m-3-3.center) -- (m-3-6.center);
  % \draw[->, thick] (m-4-4.center) -- (m-4-6.center);
  % \draw[->, thick] (m-5-5.center) -- (m-5-6.center);
  \node[n] at (a) {\textbf{a}};
}


==> src/subopt_expd.tex <==
\tikzstyle{jp}=[circle,fill=blue!40, inner sep=0pt, minimum size=4mm]
\tikzstyle{pm}=[circle,fill=cyan!50, inner sep=0pt, minimum size=4mm]
\matrix(m)[coord matrix={0.8cm}] {
  $y\backslash x$ &1&2&3&4\\
      1& & & & \\
      2& & & & \\
      3& & & & \\
      4& & & & \\
      5& & & & \\
};

\newcommand{\drawcase} {
  \node (s) at (m-3-2) [jp] {$s$};
  \node (q) at (m-6-4) [jp] {$q$};
  \node (p) at (m-2-4) [jp] {$p$};
  \node (a) at (m-3-4) [pm] {$a$};
  \draw[-, thick, blue!80, shorten <=2pt] (s.north) -- (m-2-2.center);
  \draw[->, thick, blue!80, shorten >=5pt] (m-2-2.center) -- (p.center);
  \draw[->|, thick, blue!80, shorten <= 5pt, shorten >= 5pt] ([xshift=5pt]p.center) -- ([xshift=5pt]q.center);
  \draw[-, thick, shorten <= 2pt] (s.south) -- (m-6-2.center);
  \draw[->, thick, shorten >= 5pt] (m-6-2.center) -- (q.center);
  \draw[->|, thick, shorten <= 5pt, shorten >= 5pt] (q.center) -- (a.center);

  \begin{scope}[on background layer]
    \node[fill=black, inner sep=0pt, fit=(m-3-3)(m-5-3)]{};
    \node[fill=black, inner sep=0pt, fit=(m-4-5)(m-6-5)]{};
  \end{scope}
}


